Lifted Neural Networks

We describe a novel family of models of multi- layer feedforward neural networks in which the activation functions are encoded via penalties in the training problem. Our approach is based on representing a non-decreasing activation function as the argmin of an appropriate convex optimiza- tion problem. The new framework allows for algo- rithms such as block-coordinate descent methods to be applied, in which each step is composed of a simple (no hidden layer) supervised learning problem that is parallelizable across data points and/or layers. Experiments indicate that the pro- posed models provide excellent initial guesses for weights for standard neural networks. In addi- tion, the model provides avenues for interesting extensions, such as robustness against noisy in- puts and optimizing over parameters in activation functions.

==> non_convex_datasets.tex <==
\section{RNN Dataset Description} % (fold)
\paragraph{Lag Sequence}
This is another classification task.  The input is a sequence of uniformly random values between -1 and 1.  At each time point, the output is a 1-hot vector.  The output is on (index 0 is 1) if the sum of the input values up to that point are positive.  If the sum of the values are negative, then the output is off (index 1 is 1).  The running sum, RS, is written to help illustrate the mechanics of the dataset.

\begin{align}
&x = \begin{pmatrix}
-0.26 & 0.55 & -0.78 & 0.05 & 0.89 & 0.12
\end{pmatrix} \\
&y = \begin{pmatrix}
0 & 1 & 0 & 0 & 1 & 1 \\
1 & 0 & 1 & 1 & 0 & 0
\end{pmatrix}\\
&RS = \begin{pmatrix}
-0.26 & 0.29 & -0.49 & -0.44 & 0.45 & 0.57 
\end{pmatrix}
\end{align}

\paragraph{Sum of Random Values Thresholded}
This is another classification task.  The input is a sequence of uniformly random values between -1 and 1.  At each time point, the output is a 1-hot vector.  The output is on (index 0 is 1) if the sum of the input values up to that point are positive.  If the sum of the values are negative, then the output is off (index 1 is 1).  The running sum, RS, is written to help illustrate the mechanics of the dataset.

$x = \begin{pmatrix}
-0.26 & 0.55 & -0.78 & 0.05 & 0.89 & 0.12
\end{pmatrix}$
\newline
$y = \begin{pmatrix}
0 & 1 & 0 & 0 & 1 & 1 \\
1 & 0 & 1 & 1 & 0 & 0
\end{pmatrix}$
\newline
$RS = \begin{pmatrix}
-0.26 & 0.29 & -0.49 & -0.44 & 0.45 & 0.57 
\end{pmatrix}$

\paragraph{Timer}
Here we describe a timer dataset for binary classification.  The input data is three-dimensional at each timestep.  The first input is a random integer between 1 and p inclusive.  p indicates the longest possible timer value.  This value will indicate how long our timer is on.  The second/third inputs indicates whether the on switch is on for the timer.  We imagine that there is a running timer which is a single integer.  At each time step, the running timer decreases by 1 (or if it's zero it stays at zero).  Then we consider the next input vector.  If the second input is off then we ignore that timestep input.  If the second input is on, then we update our running timer to be the max of the previous running timer and the timer input.  We specify the fraction of the time that the inputs are on as a hyperparameter.  The fraction and the actual time value are independent of each other.

The output is a two-dimensional one-hot vector at each time step.  Our output at each time point will be "on" if the running timer has a positive value and "off" if the running timer has a negative value.  The running timer labelled as RT is given here to illustrate the mechanics of the example.

$x = \begin{pmatrix}
3 & 2 & 5 & 4 & 2 & 4 \\
0 & 1 & 0 & 0 & 1 & 0 \\
1 & 0 & 1 & 1 & 0 & 1 \\
\end{pmatrix}$
\newline
$y = \begin{pmatrix}
0 & 1 & 1 & 0 & 1 & 1 \\
1 & 0 & 0 & 1 & 0 & 0
\end{pmatrix}$
\newline
$RT = \begin{pmatrix}
0 & 2 & 1 & 0 & 2 & 1 \\
\end{pmatrix}$

